High-Level Synthesis Performance Prediction using GNNs: Benchmarking, Modeling, and Advancing

Agile hardware development requires fast and accurate circuit quality evaluation from early design stages. Existing work of high-level synthesis (HLS) performance prediction usually needs extensive feature engineering after the synthesis process. To expedite circuit evaluation from as earlier design stage as possible, we propose a rapid and accurate performance modeling, exploiting the representation power of graph neural networks (GNNs) by representing C/C++ programs as graphs. The contribution of this work is three-fold. First, we build a standard benchmark containing 40k C synthesizable programs, which includes both synthetic programs and three sets of real-world HLS benchmarks. Each program is implemented on FPGA to generate ground-truth performance metrics. Second, we formally formulate the HLS performance prediction problem on graphs, and propose multiple modeling strategies with GNNs that leverage different trade-offs between prediction timeliness (early/late prediction) and accuracy. Third, we further propose a novel hierarchical GNN that does not sacrifice timeliness but largely improves prediction accuracy, significantly outperforming HLS tools. We apply extensive evaluations for both synthetic and unseen real-case programs; our proposed predictor largely outperforms HLS by up to 40X and excels existing predictors by 2X to 5X in terms of resource usage and timing prediction.

==> 0_related.tex <==
\section{Related Work}

\noindent
\textbf{ML-based HLS performance prediction.}
Pyramid~\cite{makrani2019pyramid} is one representative work that used ML models for resource and timing prediction, including linear regression, artificial neural network, support vector machine, random forest, and an ensemble model combining the four. They require 183 features extracted from HLS report.
%HL-Pow~\cite{lin2020hl} is an ML-based predictor for power modeling of HLS.
Both HLSPredict~\cite{o2018hlspredict} and XPPE~\cite{makrani2019xppe} are ANN-based cross-platform performance predictor that estimates the HLS design performance on a specific FPGA,
where HLSPredict used up to 75 features, and XPPE was extended from Pyramid for unseen FPGAs and also used 183 features.
IronMan~\cite{wu2021ironman} is a most recent work where part of it exploits GNNs for HLS performance  prediction, largely outperforming the commercial HLS tool. However it only focuses on simplest and small programs with only additions and multiplications, and thus less realistic.


\noindent
\textbf{GNNs in EDA.}
There has been signs of emergence in using GNN approaches to solving problems in EDA that can be naturally modeled as graphs.
Circuit-GNN~\cite{zhang2019circuit} uses GNNs to simulate electromagnetic (EM) properties of distributed circuits to replace traditional EM simulators.
Another category is to model the chip placement into graph formulation; the prediction goals can be wirelength or chip area for digital circuits~\cite{mirhoseini2020chip}, and gain, bandwidth, or phase margin for analog circuits~\cite{li2020customized}.
Analog circuit (transistor) sizing and symmetry annotation have also been studied~\cite{wang2020gcn, gao2021layout, chen2021universal}, where the constraints for circuit layout are automatically annotated by GNNs.
Ustun et at.~\cite{ustun2020accurate} use GNNs for operation delay prediction on FPGAs.
These prior arts demonstrate potentials of GNNs in solving EDA problems.





